Analysis of Indexing Structures for Immutable Data

In emerging applications such as blockchains and collaborative data analytics, there are strong demands for data immutability, multi-version accesses, and tamper-evident controls. This leads to three new index structures for immutable data, namely Merkle Patricia Trie (MPT), Merkle Bucket Tree (MBT), and Pattern-Oriented-Split Tree (POS-Tree). Although these structures have been adopted in real applications, there is no systematic evaluation of their pros and cons in the literature. This makes it difficult for practitioners to choose the right index structure for their applications, as there is only a limited understanding of the characteristics of each index. To alleviate the above deficiency, we present a comprehensive analysis of the existing index structures for immutable data, evaluating both their asymptotic and empirical performance. Specifically, we show that MPT, MBT, and POS-Tree are all instances of a recently proposed framework, dubbed \my{Structurally Invariant and Reusable Indexes (SIRI)}. We propose to evaluate the SIRI instances based on five essential metrics: their efficiency for four index operations (i.e., lookup, update, comparison, and merge), as well as their \my{deduplication ratios} (i.e., the size of the index with deduplication over the size without deduplication). We establish the worst-case guarantees of each index in terms of these five metrics, and we experimentally evaluate all indexes in a large variety of settings. Based on our theoretical and empirical analysis, we conclude that POS-Tree is a favorable choice for indexing immutable data.

==> sections/impl.tex <==
\section{Implementation}
\label{sec:impl}

\noindent

This section describes the implementation details of the three representatives of \myindex (Section \ref{subsec:pos-impl}, \ref{subsec:mbt-impl}, \ref{subsec:mpt-impl}) and our baseline index (Section \ref{subsec:mvmb-impl}).

\subsection{Multi-version Merkle B+ Tree}
\label{subsec:mvmb-impl}

\noindent

We first describe our baseline implementation. We target on the multi-version database context and emerging tamper-resilient demand. Therefore, traditional index structures such as B-tree family do not fit in the context. For a fair comparison between \myindex and non-\myindex, we extended B+ tree with tampler-resilience and immutability. First, we replace the pointers stored in index nodes with the hash of their immediate children and maintains an additional table from the hash to the actual address. As in \mytree, MBT and MPT, this Merkle Tree like structure enables tampler-resilience as well as provides efficient lookup for duplicate nodes. Second, instead of performing in-line updates, we make new copy of the entire node including the updates. Such implementation of immutability guarantees all versions of data can be retrieved without overhead due to locking or additional lookup. We call this modified B+ tree Multi-version Merkle B+ tree (MVMB+-Tree) in the rest of the paper.

\subsection{\mytree}
\label{subsec:pos-impl}

% \hlight{(Incomplete)}

\noindent

We use the \mytree implementation provided in Forkbase~\cite{wang:2018}. However, there are several problems making the original \mytree less efficient in both lookup and write. Firstly, it used linear scan when searching for key position. As mentioned in Section~\ref{subsec:pos}, the keys are maintained in order. Hence we replaced linear scan with binary search to improve the performance. This improvement could be significant when the number of entries in each index node is large. Secondly, the original \mytree calculated rolling hash for both meta nodes and leaf nodes, causing the data update very inefficient. With detailed breakdown analysis, the computation of rolling hash is accounted for half of the write execution time. Regarding to this problem, instead of calculating rolling hash in meta nodes, we directly search for patterns using child hash. This improvement removed redundant hash calculation and the overhead of sliding window is mitigated. Lastly, we optimize the write operation with batching techniques, which reduce the number of tree traversal and hash calculations significantly. With the improvements, \mytree could achieve performance comparable to MVMB+-Tree. 

\subsection{Merkle Bucket Tree}
\label{subsec:mbt-impl}

We implemented MBT based on source code provided in Hyperledger Fabric 0.6~\cite{web:hyperledger}. We could not use the implementation directly due to three reasons. First, the source code of Hyperledger 0.6 is only available in GO. Therefore, we migrated the code to C++. Second, MBT is not used as storage index in Hyperledger. Instead, it is mainly used to provide tamper-evidence for ledger state. The indexing is managed by underlying RocksDB. During a lookup or write, data is accessed through RocksDB API. To adapt it as a storage index, we fetch the keys by traversing the tree from the root for a lookup operation and update the data and index in bottom-up manner for a write operation. Third, the original MBT is mutable because it is used to provide tamper-evidence for state, not the ledger. Similar as MVMB+-Tree, we apply node-level copy-on-write to make the structure immutable and fit in multi-version database context.

\subsection{Merkle Patricia Trie}
\label{subsec:mpt-impl}

Lastly, we implemented a C++ version of MPT based on source code provided in Ethereum. MPT is a combination of Radix tree and Merkle tree, where each node only stores a sub-sequence of key and link between index node is maintained by hash. To make MPT efficient in both processing time and storage space. Extension node is introduced to combine the nodes on a path that only have one branch. During write operation, in case the inserting key and extension node have a partial match. New extension node with matched key sequence will be created and attached a branch node containing the first character of distinct key sequence. During a remove operation, if a branch node only contains single child, it will be removed and combined with adjacent child and parent extension nodes.

==> sections/related.tex <==
\section{Related Work}
\label{sec:relate}

\hlight{(Need Rephrase)}

\subsection{Versioning}

Data versioning has been widely employed for tolerating failures, errors and intrusions,
and for analysis of data modification history.
ElephantFS~\cite{santry:1999} is one of the first file systems with built-in multi-version support.
Later systems like S4~\cite{strunk:2000}, CVFS~\cite{soules:2003}, RepareStore~\cite{zhu:2003}
and OceanStore~\cite{kubiatowicz:2000},
improve the early design by maintaining all versions in full scope and upon each update operation.
Most of these systems use journal/log-structure file system (e.g.,
SpriteLFS~\cite{rosenblum:1992}) as the underlying storage,
because they leverage the latter's high performance in
append-only workloads.
In databases, data versioning techniques are used for transactional data access.
Postgres~\cite{stonebraker:1987, bernstein:1983}, for example, achieved
performance comparable to other database systems without versioning support.
Fastrek~\cite{chiueh:2005} enhanced
Postgres with intrusion tolerance by maintaining an inter-transaction dependency graph based on the versioned data,
and relying on the graph to resolve data access conflicts. 

\subsection{Immutability}

Data \emph{immutability} means data cannot be modified after creation.
It is widely exploited in data-oriented systems,
in which it helps facilitate data replication, consistency and failure recovery.
For example, massively parallel systems~\cite{dean:2014, isard:2007, zaharia:2010}
take immutable files from DFS~\cite{web:hdfs,ghemawat:2003} as input.
Resilient Distributed Datasets used in Spark~\cite{zaharia:2010}
are in essence immutable datasets containing operation history.
More importantly,
immutability is a fundamental concept in emerging applications,
such as blockchain platforms~\cite{web:ethereum, web:hyperledger, nakamoto:2009}.
In these applications, immutability also means \emph{tamper resistance}.
Data cannot be modified by not only application itself,
but also malicious participants or external attacks.
Any tamper of data should be able to be detected.

\subsection{Deduplication}

Maintaining massive data versions and branches is challenging,
since continuous ingestion of data modification
can rapidly lead to a volume explosion.
Hence, data \emph{deduplication} is critical to
avoid maintaining redundant data copies,
reducing storage overhead.
Data deduplication can be conducted at different granularities.
Git deduplicates data at file level,
where a single copy is kept for identical files.
Moreover, compaction is triggered periodically
to further pack similar files.
Similarly, collaborative analytic engines
deduplicate at sub-table level.
Decibel~\cite{maddox:2016} studies differences between
row/column-based schemes,
while OrpheusDB~\cite{xu:2017} applies an advanced partitioning
strategy to tune tradeoff between checkout time and space consumption.

\subsection{Oblivious Data Structures}

\hlight{(Incomplete, Need Rephrase)}

Oblivious data structures~\cite{naor:2001} (or called history independent data structures) are designed for eliminating history information
for privacy purpose.
There are two practical ways to make a data structure history independent.
One is to ensure that the representation of the structure is determined by its current content 
--- for example, an array of elements can be kept in a history independent way
by sorting the elements and always placing them as close to the 0-th cell as possible.
Then the array's contents are exactly the current elements in sorted order,
arranged at the beginning of the table,
regardless of their insertion (or deletion) order.
The second way is to introduce secret randomness into the data structure in such a way that an observer who does not know the random choices cannot infer anything about the history.
An example of this is storing elements in an array in some order which is a random permutation of their insertion order,
where the permutation is secret and never stored explicitly.

Oblivious data structures exactly fulfil the \textit{Structurally Invariant} property of \myindex.
